A Benchmark for Localizing Code and Non-Code Issues in Software Projects

Accurate project localization (e.g., files and functions) for issue resolution is a critical first step in software maintenance. However, existing benchmarks for issue localization, such as SWE-Bench and LocBench, are limited. They focus predominantly on pull-request issues and code locations, ignoring other evidence and non-code files such as commits, comments, configurations, and documentation. To address this gap, we introduce MULocBench, a comprehensive dataset of 1,100 issues from 46 popular GitHub Python projects. Comparing with existing benchmarks, MULocBench offers greater diversity in issue types, root causes, location scopes, and file types, providing a more realistic testbed for evaluation. Using this benchmark, we assess the performance of state-of-the-art localization methods and five LLM-based prompting strategies. Our results reveal significant limitations in current techniques: even at the file level, performance metrics (Acc@5, F1) remain below 40%. This underscores the challenge of generalizing to realistic, multi-faceted issue resolution. To enable future research on project localization for issue resolution, we publicly release MULocBench at https://huggingface.co/datasets/somethingone/MULocBench.

==> dsl_stat.tex <==

\begin{table}[h]
\label{tab:dsl}
\centering
\scalebox{0.85}{
\begin{tabular}{clllllll}
\multicolumn{1}{c}{\cellcolor[gray]{0.9}}&
\multicolumn{1}{|c|}{\cellcolor[gray]{0.9}Name}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}\#Rule}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}\#DSL}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Acc(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}P(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}R(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}F(\%)}\\ \hline


\multirow{2}{*}{Coding Standard}&
\multicolumn{1}{|c|}{Google Java Style Guide}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}\\
\cline{2-8}&
\multicolumn{1}{|c|}{Google JavaScript Style Guide}&
\multicolumn{1}{c}{108}&
\multicolumn{1}{c}{394}&
\multicolumn{1}{c}{74.1}&
\multicolumn{1}{c}{90.6}&
\multicolumn{1}{c}{99.4}&
\multicolumn{1}{c}{94.8}\\ \hline


\multirow{2}{*}{Tool}&
\multicolumn{1}{|c|}{Checkstyle}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}\\
\cline{2-8}&
\multicolumn{1}{|c|}{ESLint}&
\multicolumn{1}{c}{166}&
\multicolumn{1}{c}{528(basic 304)}&
\multicolumn{1}{c}{78.3}&
\multicolumn{1}{c}{87.4}&
\multicolumn{1}{c}{99.4}&
\multicolumn{1}{c}{93.0}\\ \hline

\end{tabular}
}

\end{table}


==> evaluation_improvement.tex <==
\noindent \textbf{Note:}   Underlined values indicate the best performance among the baselines. Bold values represent the best performance across all methods. "Improvement" indicates the minimum improvement over the baselines. For baselines that cannot be run due to token limits, results are marked with '-'.


\begin{table}[h]
\scriptsize\caption{Results of Generating Checkstyle Configuration for Google Java Style Guide.}
  \label{tab:checkstyle_result_table}
  \vspace{-0.1cm}
\centering
\scalebox{0.8}{
\begin{tabular}{|c|llllllllllll|}
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{|c|}{Rule Name} &
\multicolumn{4}{|c|}{Option Name} &
\multicolumn{4}{|c|}{Option Value} \\
\cline{2-13} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} \\ \hline

\multicolumn{1}{|c|}{closed book}&\multicolumn{1}{|c|}{38.2}&\multicolumn{1}{|c|}{\underline{39.4}}&\multicolumn{1}{|c|}{58.6}&\multicolumn{1}{|c|}{\underline{47.1}}&\multicolumn{1}{|c|}{20.6}&\multicolumn{1}{|c|}{24.0}&\multicolumn{1}{|c|}{35.7}&\multicolumn{1}{|c|}{28.7}&\multicolumn{1}{|c|}{33.8}&\multicolumn{1}{|c|}{\underline{28.8}}&\multicolumn{1}{|c|}{42.9}&\multicolumn{1}{|c|}{\underline{34.5}}\\ \hline

\multicolumn{1}{|c|}{name}&\multicolumn{1}{|c|}{42.6}&\multicolumn{1}{|c|}{17.1}&\multicolumn{1}{|c|}{81.2}&\multicolumn{1}{|c|}{28.3}&\multicolumn{1}{|c|}{23.5}&\multicolumn{1}{|c|}{11.3}&\multicolumn{1}{|c|}{53.6}&\multicolumn{1}{|c|}{18.7}&\multicolumn{1}{|c|}{33.8}&\multicolumn{1}{|c|}{12.5}&\multicolumn{1}{|c|}{59.4}&\multicolumn{1}{|c|}{20.7}\\ \hline

\multicolumn{1}{|c|}{name\_desc}&\multicolumn{1}{|c|}{44.1}&\multicolumn{1}{|c|}{25.7}&\multicolumn{1}{|c|}{80.9}&\multicolumn{1}{|c|}{39.0}&\multicolumn{1}{|c|}{29.4}&\multicolumn{1}{|c|}{20.1}&\multicolumn{1}{|c|}{63.2}&\multicolumn{1}{|c|}{30.5}&\multicolumn{1}{|c|}{30.9}&\multicolumn{1}{|c|}{17.3}&\multicolumn{1}{|c|}{54.4}&\multicolumn{1}{|c|}{26.2}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt}&\multicolumn{1}{|c|}{\underline{51.5}}&\multicolumn{1}{|c|}{23.4}&\multicolumn{1}{|c|}{\textbf{\underline{84.1}}}&\multicolumn{1}{|c|}{36.6}&\multicolumn{1}{|c|}{\underline{51.5}}&\multicolumn{1}{|c|}{23.0}&\multicolumn{1}{|c|}{\textbf{\underline{82.6}}}&\multicolumn{1}{|c|}{36.0}&\multicolumn{1}{|c|}{\underline{39.7}}&\multicolumn{1}{|c|}{17.7}&\multicolumn{1}{|c|}{\underline{63.8}}&\multicolumn{1}{|c|}{27.8}\\ \hline

\multicolumn{1}{|c|}{name\_desc (RAG)}&\multicolumn{1}{|c|}{16.2}&\multicolumn{1}{|c|}{23.5}&\multicolumn{1}{|c|}{77.6}&\multicolumn{1}{|c|}{36.1}&\multicolumn{1}{|c|}{14.7}&\multicolumn{1}{|c|}{20.4}&\multicolumn{1}{|c|}{67.2}&\multicolumn{1}{|c|}{31.2}&\multicolumn{1}{|c|}{13.2}&\multicolumn{1}{|c|}{16.3}&\multicolumn{1}{|c|}{53.7}&\multicolumn{1}{|c|}{25.0}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt (RAG)}&\multicolumn{1}{|c|}{25.0}&\multicolumn{1}{|c|}{31.8}&\multicolumn{1}{|c|}{79.4}&\multicolumn{1}{|c|}{45.4}&\multicolumn{1}{|c|}{25.0}&\multicolumn{1}{|c|}{\underline{31.8}}&\multicolumn{1}{|c|}{79.4}&\multicolumn{1}{|c|}{\underline{45.4}}&\multicolumn{1}{|c|}{13.2}&\multicolumn{1}{|c|}{17.6}&\multicolumn{1}{|c|}{44.1}&\multicolumn{1}{|c|}{25.2}\\ \hline

\multicolumn{1}{|c|}{\textbf{Our Method}}&\multicolumn{1}{|c|}{\textbf{81.2}}&\multicolumn{1}{|c|}{\textbf{92.1}}&\multicolumn{1}{|c|}{\textbf{\underline{84.1}}}&\multicolumn{1}{|c|}{\textbf{87.9}}&\multicolumn{1}{|c|}{\textbf{78.3}}&\multicolumn{1}{|c|}{\textbf{84.1}}&\multicolumn{1}{|c|}{76.8}&\multicolumn{1}{|c|}{\textbf{80.3}}&\multicolumn{1}{|c|}{\textbf{76.8}}&\multicolumn{1}{|c|}{\textbf{76.2}}&\multicolumn{1}{|c|}{\textbf{69.6}}&\multicolumn{1}{|c|}{\textbf{72.7}}\\ \hline

\multicolumn{1}{|c|}{Improvement}&\multicolumn{1}{|c|}{57.7}&\multicolumn{1}{|c|}{133.8}&\multicolumn{1}{|c|}{0.0}&\multicolumn{1}{|c|}{86.6}&\multicolumn{1}{|c|}{52.0}&\multicolumn{1}{|c|}{164.5}&\multicolumn{1}{|c|}{-7.0}&\multicolumn{1}{|c|}{76.9}&\multicolumn{1}{|c|}{93.5}&\multicolumn{1}{|c|}{164.6}&\multicolumn{1}{|c|}{9.1}&\multicolumn{1}{|c|}{110.7}\\ \hline


\end{tabular}
}
\vspace{-0.2cm}
\end{table}


\begin{table}[h]
\scriptsize\caption{Results of Generating ESLint Configuration for Google JavaScript Style Guide.}
  \label{tab:ESLint_result_table}
  \vspace{-0.1cm}
\centering
\scalebox{0.8}{
\begin{tabular}{|c|llllllllllll|}
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{|c|}{Rule Name} &
\multicolumn{4}{|c|}{Option Name} &
\multicolumn{4}{|c|}{Option Value} \\
\cline{2-13} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} \\ \hline

\multicolumn{1}{|c|}{closed book}&\multicolumn{1}{|c|}{27.5}&\multicolumn{1}{|c|}{15.5}&\multicolumn{1}{|c|}{65.1}&\multicolumn{1}{|c|}{25.1}&\multicolumn{1}{|c|}{24.8}&\multicolumn{1}{|c|}{11.8}&\multicolumn{1}{|c|}{49.4}&\multicolumn{1}{|c|}{19.0}&\multicolumn{1}{|c|}{24.8}&\multicolumn{1}{|c|}{10.1}&\multicolumn{1}{|c|}{42.2}&\multicolumn{1}{|c|}{16.2}\\ \hline

\multicolumn{1}{|c|}{name}&\multicolumn{1}{|c|}{18.8}&\multicolumn{1}{|c|}{10.5}&\multicolumn{1}{|c|}{83.1}&\multicolumn{1}{|c|}{18.6}&\multicolumn{1}{|c|}{16.1}&\multicolumn{1}{|c|}{7.6}&\multicolumn{1}{|c|}{60.2}&\multicolumn{1}{|c|}{13.5}&\multicolumn{1}{|c|}{16.1}&\multicolumn{1}{|c|}{7.0}&\multicolumn{1}{|c|}{55.4}&\multicolumn{1}{|c|}{12.4}\\ \hline

\multicolumn{1}{|c|}{name\_desc}&\multicolumn{1}{|c|}{\underline{32.2}}&\multicolumn{1}{|c|}{\underline{20.8}}&\multicolumn{1}{|c|}{72.3}&\multicolumn{1}{|c|}{\underline{32.3}}&\multicolumn{1}{|c|}{\underline{28.2}}&\multicolumn{1}{|c|}{\underline{15.3}}&\multicolumn{1}{|c|}{53.0}&\multicolumn{1}{|c|}{\underline{23.7}}&\multicolumn{1}{|c|}{\underline{27.5}}&\multicolumn{1}{|c|}{\underline{14.2}}&\multicolumn{1}{|c|}{49.4}&\multicolumn{1}{|c|}{\underline{22.1}}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}\\ \hline

\multicolumn{1}{|c|}{name\_desc (RAG)}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{9.2}&\multicolumn{1}{|c|}{79.5}&\multicolumn{1}{|c|}{16.5}&\multicolumn{1}{|c|}{10.7}&\multicolumn{1}{|c|}{6.4}&\multicolumn{1}{|c|}{55.4}&\multicolumn{1}{|c|}{11.5}&\multicolumn{1}{|c|}{10.7}&\multicolumn{1}{|c|}{6.0}&\multicolumn{1}{|c|}{51.8}&\multicolumn{1}{|c|}{10.8}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt (RAG)}&\multicolumn{1}{|c|}{16.8}&\multicolumn{1}{|c|}{7.8}&\multicolumn{1}{|c|}{\textbf{\underline{85.5}}}&\multicolumn{1}{|c|}{14.4}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{5.7}&\multicolumn{1}{|c|}{\textbf{\underline{62.7}}}&\multicolumn{1}{|c|}{10.5}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{5.4}&\multicolumn{1}{|c|}{\underline{59.0}}&\multicolumn{1}{|c|}{9.9}\\ \hline

\multicolumn{1}{|c|}{Our Method}&\multicolumn{1}{|c|}{\textbf{83.1}}&\multicolumn{1}{|c|}{\textbf{83.9}}&\multicolumn{1}{|c|}{67.5}&\multicolumn{1}{|c|}{\textbf{74.8}}&\multicolumn{1}{|c|}{\textbf{79.6}}&\multicolumn{1}{|c|}{\textbf{75.8}}&\multicolumn{1}{|c|}{61.0}&\multicolumn{1}{|c|}{\textbf{67.6}}&\multicolumn{1}{|c|}{\textbf{79.6}}&\multicolumn{1}{|c|}{\textbf{74.2}}&\multicolumn{1}{|c|}{\textbf{59.7}}&\multicolumn{1}{|c|}{\textbf{66.2}}\\ \hline

\multicolumn{1}{|c|}{Improvement}&\multicolumn{1}{|c|}{158.1}&\multicolumn{1}{|c|}{303.4}&\multicolumn{1}{|c|}{-21.1}&\multicolumn{1}{|c|}{131.6}&\multicolumn{1}{|c|}{182.3}&\multicolumn{1}{|c|}{395.4}&\multicolumn{1}{|c|}{-2.7}&\multicolumn{1}{|c|}{185.2}&\multicolumn{1}{|c|}{189.5}&\multicolumn{1}{|c|}{422.5}&\multicolumn{1}{|c|}{1.2}&\multicolumn{1}{|c|}{199.5}\\ \hline

\end{tabular}
}
\vspace{-0.2cm}
\end{table}


==> evaluation_improvement2.tex <==


\begin{table}[h]
\label{tab:gen_config_result_table}
\centering
\scalebox{0.75}{
\begin{tabular}{c|llllllllllll|}



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating Java Configuration for Google Checkstyle Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Rule Name-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{38.2}&\multicolumn{1}{c}{\underline{39.4}}&\multicolumn{1}{c}{58.6}&\multicolumn{1}{c}{\underline{47.1}}&\multicolumn{1}{|c}{20.6}&\multicolumn{1}{c}{24.0}&\multicolumn{1}{c}{35.7}&\multicolumn{1}{c}{28.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{\underline{28.8}}&\multicolumn{1}{c}{42.9}&\multicolumn{1}{c}{\underline{34.5}}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{42.6}&\multicolumn{1}{c}{17.1}&\multicolumn{1}{c}{81.2}&\multicolumn{1}{c}{28.3}&\multicolumn{1}{|c}{23.5}&\multicolumn{1}{c}{11.3}&\multicolumn{1}{c}{53.6}&\multicolumn{1}{c}{18.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{12.5}&\multicolumn{1}{c}{59.4}&\multicolumn{1}{c}{20.7}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{44.1}&\multicolumn{1}{c}{25.7}&\multicolumn{1}{c}{80.9}&\multicolumn{1}{c}{39.0}&\multicolumn{1}{|c}{29.4}&\multicolumn{1}{c}{20.1}&\multicolumn{1}{c}{63.2}&\multicolumn{1}{c}{30.5}&\multicolumn{1}{|c}{30.9}&\multicolumn{1}{c}{17.3}&\multicolumn{1}{c}{54.4}&\multicolumn{1}{c}{26.2}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.4}&\multicolumn{1}{c}{\textbf{\underline{84.1}}}&\multicolumn{1}{c}{36.6}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.0}&\multicolumn{1}{c}{\textbf{\underline{82.6}}}&\multicolumn{1}{c}{36.0}&\multicolumn{1}{|c}{\underline{39.7}}&\multicolumn{1}{c}{17.7}&\multicolumn{1}{c}{\underline{63.8}}&\multicolumn{1}{c}{27.8}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{16.2}&\multicolumn{1}{c}{23.5}&\multicolumn{1}{c}{77.6}&\multicolumn{1}{c}{36.1}&\multicolumn{1}{|c}{14.7}&\multicolumn{1}{c}{20.4}&\multicolumn{1}{c}{67.2}&\multicolumn{1}{c}{31.2}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{16.3}&\multicolumn{1}{c}{53.7}&\multicolumn{1}{c}{25.0}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{31.8}&\multicolumn{1}{c}{79.4}&\multicolumn{1}{c}{45.4}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{\underline{31.8}}&\multicolumn{1}{c}{79.4}&\multicolumn{1}{c}{\underline{45.4}}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{17.6}&\multicolumn{1}{c}{44.1}&\multicolumn{1}{c}{25.2}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{81.2}}&\multicolumn{1}{c}{\textbf{92.1}}&\multicolumn{1}{c}{\textbf{\underline{84.1}}}&\multicolumn{1}{c}{\textbf{87.9}}&\multicolumn{1}{|c}{\textbf{78.3}}&\multicolumn{1}{c}{\textbf{84.1}}&\multicolumn{1}{c}{76.8}&\multicolumn{1}{c}{\textbf{80.3}}&\multicolumn{1}{|c}{\textbf{76.8}}&\multicolumn{1}{c}{\textbf{76.2}}&\multicolumn{1}{c}{\textbf{69.6}}&\multicolumn{1}{c}{\textbf{72.7}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{57.7}&\multicolumn{1}{c}{133.8}&\multicolumn{1}{c}{0.0}&\multicolumn{1}{c}{86.6}&\multicolumn{1}{|c}{52.0}&\multicolumn{1}{c}{164.5}&\multicolumn{1}{c}{-7.0}&\multicolumn{1}{c}{76.9}&\multicolumn{1}{|c}{93.5}&\multicolumn{1}{c}{164.6}&\multicolumn{1}{c}{9.1}&\multicolumn{1}{c}{110.7}\\ \hline



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating JavaScript Configuration for Google ESLint Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Rule Name-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{27.5}&\multicolumn{1}{c}{15.5}&\multicolumn{1}{c}{65.1}&\multicolumn{1}{c}{25.1}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{11.8}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{19.0}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{10.1}&\multicolumn{1}{c}{42.2}&\multicolumn{1}{c}{16.2}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{18.8}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{c}{83.1}&\multicolumn{1}{c}{18.6}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.6}&\multicolumn{1}{c}{60.2}&\multicolumn{1}{c}{13.5}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.0}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{12.4}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{\underline{32.2}}&\multicolumn{1}{c}{\underline{20.8}}&\multicolumn{1}{c}{72.3}&\multicolumn{1}{c}{\underline{32.3}}&\multicolumn{1}{|c}{\underline{28.2}}&\multicolumn{1}{c}{\underline{15.3}}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{\underline{23.7}}&\multicolumn{1}{|c}{\underline{27.5}}&\multicolumn{1}{c}{\underline{14.2}}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{\underline{22.1}}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{9.2}&\multicolumn{1}{c}{79.5}&\multicolumn{1}{c}{16.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.4}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{11.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.0}&\multicolumn{1}{c}{51.8}&\multicolumn{1}{c}{10.8}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{16.8}&\multicolumn{1}{c}{7.8}&\multicolumn{1}{c}{\textbf{\underline{85.5}}}&\multicolumn{1}{c}{14.4}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.7}&\multicolumn{1}{c}{\textbf{\underline{62.7}}}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.4}&\multicolumn{1}{c}{\underline{59.0}}&\multicolumn{1}{c}{9.9}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{83.1}}&\multicolumn{1}{c}{\textbf{83.9}}&\multicolumn{1}{c}{67.5}&\multicolumn{1}{c}{\textbf{74.8}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{75.8}}&\multicolumn{1}{c}{61.0}&\multicolumn{1}{c}{\textbf{67.6}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{74.2}}&\multicolumn{1}{c}{\textbf{59.7}}&\multicolumn{1}{c}{\textbf{66.2}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{158.1}&\multicolumn{1}{c}{303.4}&\multicolumn{1}{c}{-21.1}&\multicolumn{1}{c}{131.6}&\multicolumn{1}{|c}{182.3}&\multicolumn{1}{c}{395.4}&\multicolumn{1}{c}{-2.7}&\multicolumn{1}{c}{185.2}&\multicolumn{1}{|c}{189.5}&\multicolumn{1}{c}{422.5}&\multicolumn{1}{c}{1.2}&\multicolumn{1}{c}{199.5}\\ \hline

\end{tabular}
}
\end{table}



==> evaluation_improvement2_newdata.tex <==


\begin{table}[h]
\label{tab:gen_config_result_table}
\centering
\scalebox{0.75}{
\begin{tabular}{c|llllllllllll|}



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating Java Configuration for Google Checkstyle Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Module-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{38.2}&\multicolumn{1}{c}{\underline{38.5}}&\multicolumn{1}{c}{58.0}&\multicolumn{1}{c}{\underline{46.2}}&\multicolumn{1}{|c}{20.6}&\multicolumn{1}{c}{23.1}&\multicolumn{1}{c}{34.8}&\multicolumn{1}{c}{27.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{\underline{27.9}}&\multicolumn{1}{c}{42.0}&\multicolumn{1}{c}{\underline{33.5}}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{42.6}&\multicolumn{1}{c}{16.8}&\multicolumn{1}{c}{80.9}&\multicolumn{1}{c}{27.8}&\multicolumn{1}{|c}{23.5}&\multicolumn{1}{c}{11.0}&\multicolumn{1}{c}{52.9}&\multicolumn{1}{c}{18.2}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{12.2}&\multicolumn{1}{c}{58.8}&\multicolumn{1}{c}{20.3}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{44.1}&\multicolumn{1}{c}{25.2}&\multicolumn{1}{c}{80.6}&\multicolumn{1}{c}{38.4}&\multicolumn{1}{|c}{29.4}&\multicolumn{1}{c}{19.6}&\multicolumn{1}{c}{62.7}&\multicolumn{1}{c}{29.9}&\multicolumn{1}{|c}{30.9}&\multicolumn{1}{c}{16.8}&\multicolumn{1}{c}{53.7}&\multicolumn{1}{c}{25.6}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.0}&\multicolumn{1}{c}{\textbf{\underline{83.8}}}&\multicolumn{1}{c}{36.1}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{22.6}&\multicolumn{1}{c}{\textbf{\underline{82.4}}}&\multicolumn{1}{c}{35.4}&\multicolumn{1}{|c}{\underline{39.7}}&\multicolumn{1}{c}{17.3}&\multicolumn{1}{c}{\underline{63.2}}&\multicolumn{1}{c}{27.2}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{16.2}&\multicolumn{1}{c}{23.1}&\multicolumn{1}{c}{77.3}&\multicolumn{1}{c}{35.5}&\multicolumn{1}{|c}{14.7}&\multicolumn{1}{c}{19.9}&\multicolumn{1}{c}{66.7}&\multicolumn{1}{c}{30.7}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{15.8}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{24.4}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{31.2}&\multicolumn{1}{c}{79.1}&\multicolumn{1}{c}{44.7}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{\underline{31.2}}&\multicolumn{1}{c}{79.1}&\multicolumn{1}{c}{\underline{44.7}}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{17.6}&\multicolumn{1}{c}{44.8}&\multicolumn{1}{c}{25.3}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{79.7}}&\multicolumn{1}{c}{\textbf{90.5}}&\multicolumn{1}{c}{\textbf{\underline{83.8}}}&\multicolumn{1}{c}{\textbf{87.0}}&\multicolumn{1}{|c}{\textbf{76.8}}&\multicolumn{1}{c}{\textbf{82.5}}&\multicolumn{1}{c}{76.5}&\multicolumn{1}{c}{\textbf{79.4}}&\multicolumn{1}{|c}{\textbf{75.4}}&\multicolumn{1}{c}{\textbf{74.6}}&\multicolumn{1}{c}{\textbf{69.1}}&\multicolumn{1}{c}{\textbf{71.8}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{54.8}&\multicolumn{1}{c}{135.1}&\multicolumn{1}{c}{0.0}&\multicolumn{1}{c}{88.3}&\multicolumn{1}{|c}{49.1}&\multicolumn{1}{c}{164.4}&\multicolumn{1}{c}{-7.2}&\multicolumn{1}{c}{77.6}&\multicolumn{1}{|c}{89.9}&\multicolumn{1}{c}{167.4}&\multicolumn{1}{c}{9.3}&\multicolumn{1}{c}{114.3}\\ \hline



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating JavaScript Configuration for Google ESLint Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Module-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{27.5}&\multicolumn{1}{c}{15.5}&\multicolumn{1}{c}{65.1}&\multicolumn{1}{c}{25.1}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{11.8}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{19.0}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{10.1}&\multicolumn{1}{c}{42.2}&\multicolumn{1}{c}{16.2}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{18.8}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{c}{83.1}&\multicolumn{1}{c}{18.6}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.6}&\multicolumn{1}{c}{60.2}&\multicolumn{1}{c}{13.5}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.0}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{12.4}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{\underline{32.2}}&\multicolumn{1}{c}{\underline{20.8}}&\multicolumn{1}{c}{72.3}&\multicolumn{1}{c}{\underline{32.3}}&\multicolumn{1}{|c}{\underline{28.2}}&\multicolumn{1}{c}{\underline{15.3}}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{\underline{23.7}}&\multicolumn{1}{|c}{\underline{27.5}}&\multicolumn{1}{c}{\underline{14.2}}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{\underline{22.1}}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{9.2}&\multicolumn{1}{c}{79.5}&\multicolumn{1}{c}{16.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.4}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{11.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.0}&\multicolumn{1}{c}{51.8}&\multicolumn{1}{c}{10.8}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{16.8}&\multicolumn{1}{c}{7.8}&\multicolumn{1}{c}{\textbf{\underline{85.5}}}&\multicolumn{1}{c}{14.4}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.7}&\multicolumn{1}{c}{\textbf{\underline{62.7}}}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.4}&\multicolumn{1}{c}{\underline{59.0}}&\multicolumn{1}{c}{9.9}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{83.1}}&\multicolumn{1}{c}{\textbf{83.9}}&\multicolumn{1}{c}{67.5}&\multicolumn{1}{c}{\textbf{74.8}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{75.8}}&\multicolumn{1}{c}{61.0}&\multicolumn{1}{c}{\textbf{67.6}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{74.2}}&\multicolumn{1}{c}{\textbf{59.7}}&\multicolumn{1}{c}{\textbf{66.2}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{158.1}&\multicolumn{1}{c}{303.4}&\multicolumn{1}{c}{-21.1}&\multicolumn{1}{c}{131.6}&\multicolumn{1}{|c}{182.3}&\multicolumn{1}{c}{395.4}&\multicolumn{1}{c}{-2.7}&\multicolumn{1}{c}{185.2}&\multicolumn{1}{|c}{189.5}&\multicolumn{1}{c}{422.5}&\multicolumn{1}{c}{1.2}&\multicolumn{1}{c}{199.5}\\ \hline

\end{tabular}
}
\end{table}



==> exp_stat.tex <==
\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Coding Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Coding Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of RuleNames} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline

\end{tabular}
}

\end{table}


\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline
\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|l|}{Coding Standard} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
% \hline
\cline{2-4} &
\multicolumn{1}{|l|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{89}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Config with Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Config with RuleName and Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Config with Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}

\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Code Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Code Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Modules} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline


\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|l|}{Code Std} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
% \hline
\cline{2-4} &
\multicolumn{1}{|l|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{80}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{RuleName with Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}


\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Code Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Code Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Modules} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline


\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|c|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{89}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|c|}{Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{RuleName with Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}

